ABC-GS: Alignment-Based Controllable Style Transfer for 3D Gaussian Splatting

3D scene stylization approaches based on Neural Radiance Fields (NeRF) achieve promising results by optimizing with Nearest Neighbor Feature Matching (NNFM) loss. However, NNFM loss does not consider global style information. In addition, the implicit representation of NeRF limits their fine-grained control over the resulting scenes. In this paper, we introduce ABC-GS, a novel framework based on 3D Gaussian Splatting to achieve high-quality 3D style transfer. To this end, a controllable matching stage is designed to achieve precise alignment between scene content and style features through segmentation masks. Moreover, a style transfer loss function based on feature alignment is proposed to ensure that the outcomes of style transfer accurately reflect the global style of the reference image. Furthermore, the original geometric information of the scene is preserved with the depth loss and Gaussian regularization terms. Extensive experiments show that our ABC-GS provides controllability of style transfer and achieves stylization results that are more faithfully aligned with the global style of the chosen artistic reference. Our homepage is available at https://vpx-ecnu.github.io/ABC-GS-website.

==> abstract.tex <==
%Ideally, objects of the same semantic class conform to the same low-dimensional manifold, and a limited 3D scene can be described as a multi-manifold distribution. Assuming that the features of the same semantic region in images follow the same manifold, the correspondence between semantics and manifolds can be extended to the image features subspace. Based on this assumption, we propose ART-Gaussian, which combines semantic information to achieve precise and controllable 3D style transfer. 

%Previous 3D stylization methods mostly rely on Neural Radiance Fields (NeRF), where the implicit representation limits fine-grained control over scene stylization.

3D scene stylization aims to modify the appearance of scenes to embody specific artistic styles. Recent approaches based on Neural Radiance Fields (NeRF) achieve very promising results by optimizing with Nearest Neighbor Feature Matching (NNFM) loss. However, NNFM loss does not consider the relationships between pixels in the feature maps of the rendered images, which makes the method only transfer a limited subset of style features and degrade the performance.
% identified as nearest neighbors in the style feature maps. 
In addition, the implicit representation of NeRF limits their fine-grained control over the resulting scenes. 
In this paper, we introduce ABC-GS, a novel framework based on 3D Gaussian Splatting to achieve high-quality 3D style transfer with real-time rendering and strict multi-view consistency. To this end, a controllable matching stage is designed to achieve precise alignment between scene content and style features through segmentation masks. Moreover, a style transfer loss function based on feature alignment is proposed to ensure that the outcomes of style transfer accurately reflect the global style of the reference image. Furthermore, the original geometric information of the scene is preserved with the depth loss and Gaussian regularization terms. Extensive experiments show that our ABC-GS provides controllability of style transfer and achieves consistent stylization results that are more faithfully aligned with the global style of the chosen artistic reference.

% Extensive experiments show that ABC-Gaussian provides controllability of style transfer and achieves high-quality stylization results that are faithful to the complete style image while maintaining real-time rendering and strict multi-view consistency.


%为了解决当前的问题，我们提出了ART-Gaussian,一种基于3dgs的新颖的3d风格迁移框架。利用高斯的显式特性，用户可以灵活进行场景内容和风格区域的匹配。同时，我们提出了一种基于特征对齐的风格迁移损失函数，能够使风格迁移结果忠实于风格图像的全局风格。此外，我们引入了深度损失和高斯正则化项来维持场景的原始几何信息。
